Neural3Points: Learning to Generate Physically Realistic Full-body Motion for Virtual Reality Users

Animating an avatar that reflects a user's action in the VR world enables natural interactions with the virtual environment. It has the potential to allow remote users to communicate and collaborate in a way as if they met in person. However, a typical VR system provides only a very sparse set of up to three positional sensors, including a head-mounted display (HMD) and optionally two hand-held controllers, making the estimation of the user's full-body movement a difficult problem. In this work, we present a data-driven physics-based method for predicting the realistic full-body movement of the user according to the transformations of these VR trackers and simulating an avatar character to mimic such user actions in the virtual world in real-time. We train our system using reinforcement learning with carefully designed pretraining processes to ensure the success of the training and the quality of the simulation. We demonstrate the effectiveness of the method with an extensive set of examples.

==> content/0_article_info.tex <==

%CCS
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10010147.10010371.10010352.10010379</concept_id>
       <concept_desc>Computing methodologies~Physical simulation</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010371.10010387.10010866</concept_id>
       <concept_desc>Computing methodologies~Virtual reality</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010371.10010352.10010378</concept_id>
       <concept_desc>Computing methodologies~Procedural animation</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010371.10010352.10010238</concept_id>
       <concept_desc>Computing methodologies~Motion capture</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Physical simulation}
\ccsdesc[500]{Computing methodologies~Virtual reality}
\ccsdesc[500]{Theory of computation~Reinforcement Learning}
\ccsdesc[300]{Computing methodologies~Motion capture}

%keywords
\keywords{three-point tracking, motion generation, reinforcement learning}

==> content/0_authors.tex <==

% Authors.
\author{Yongjing Ye}
\authornote{Both authors contributed equally to this research.}
\affiliation{%
  \institution{Chinese Academy of Sciences}%
  \city{Beijing}%
  \country{China}%
  }
\email{br-s@gmail.com}

\author{Libin Liu}
\orcid{0000-0003-2280-6817}
\authornotemark[1]
\authornote{The research was partially conducted at DeepMotion Inc., 
    and Libin Liu is currently with Center on Frontiers of Computing Studies (CFCS), Peking University}
\affiliation{%
  \institution{Peking University}%
  \department{CFCS}
  \city{Beijing}%
  \country{China}%
  }
\affiliation{%
  \institution{DeepMotion Inc.}%
  \city{San Mateo}%
  \country{USA}%
  }
\email{libin.liu@pku.edu.cn}

\author{Shihong Xia}
\affiliation{%
  \institution{Chinese Academy of Sciences}%
  \city{Beijing}%
  \country{China}%
  }
\email{badeeri@mathworks.com}

% This command defines the author string for running heads.
% \renewcommand{\shortauthors}{DeJohnette, Rowland-Smith, Badeeri, and Foyt}
\renewcommand{\shortauthors}{Ye, Liu, and Xia}


==> content/4_tracker_position_corrector.tex <==




==> content/_template_args.tex <==

%% NOTE that a single column version may be required for 
%% submission and peer review. This can be done by changing
%% the \doucmentclass[...]{acmart} in this template to 
%% \documentclass[manuscript,screen]{acmart}
%% 
%% To ensure 100% compatibility, please check the white list of
%% approved LaTeX packages to be used with the Master Article Template at
%% https://www.acm.org/publications/taps/whitelist-of-latex-packages 
%% before creating your document. The white list page provides 
%% information on how to submit additional LaTeX packages for 
%% review and adoption.
%% Fonts used in the template cannot be substituted; margin 
%% adjustments are not allowed.
%%
%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
%\setcopyright{acmcopyright}
%\copyrightyear{2022}
%\acmYear{2022}
%\acmDOI{10.1145/1122445.1122456}

%% These commands are for a PROCEEDINGS abstract or paper.
%\acmConference[SIGGRAPH '22]{SIGGRAPH 2022}{June 03--05, 2021}{Virtual Event}
%% \acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection,
%% June 03--05, 2018, Woodstock, NY}
%\acmPrice{15.00}
%\acmISBN{978-1-4503-XXXX-X/18/06}


%%
%% Submission ID.
%% Use this when submitting an article to a sponsored event. You'll
%% receive a unique submission ID from the organizers
%% of the event, and this ID should be used as the parameter to this command.
\acmSubmissionID{270}

%%
%% The majority of ACM publications use numbered citations and
%% references.  The command \citestyle{authoryear} switches to the
%% "author year" style.
%%
%% If you are preparing content for an event
%% sponsored by ACM SIGGRAPH, you must use the "author year" style of
%% citations and references.
%% Uncommenting
%% the next command will enable that style.
\citestyle{acmauthoryear}
% \setcitestyle{square}

% A useful command for controlling the number of authors per row.
% The default value of "authorsperrow" is 2.
% \settopmatter{authorsperrow=4}

==> content/xx_high-level_policy.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{High-level Policies}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Training with simulation
\subsection{Locomotion Tasks}
\subsection{Push-recovery}
\subsection{Upper-body Control}
\subsection{3-point Tracking}


==> content/xx_introduction.tex <==

\section{Introduction}
\label{sec:introduction}

Animating an avatar in the virtual reality (VR) world that can reproduce a user's motion allows a user to see 

provides an immersive experience and enables many potential interactions and applications. 

However, a typical VR system only provides up to three trackers, including a head-mounted display (HMD) and optionally two hand-held controllers, making the estimation of the user's full-body movement a difficult problem. In this work, we present a data-driven physics-based method for predicting realistic full-body movement of the user according to the transformations of these VR trackers and simulating an avatar character to mimic such user actions in the virtual world at real-time. We train our system using reinforcement learning with carefully designed pretraining processes to ensure the success of the training and the quality of the simulation. We demonstrate the effectiveness of the method with an extensive set of examples.


Creating physics-based characters that can move freely and interact with the environment has been a long-standing computer graphics topic. Designing correct control strategies to maintain balance and travel in the environment is a notoriously difficult problem. Data-driven approaches have recently been demonstrated to be a promising way to address this issue. By combining the power of generative models and reinforcement learning, several recent works achieve interactive simulation of multiple locomotion skills.

A few problems of those recent data-driven approaches:

\begin{itemize}
    \item Many existing works rely on generative models to deal with unseen situations. 
    Those models are usually trained offline with data, but it is hard to train such models to handle dynamic interactions, such as push-recovery, without simulation.
    \item They rely on a comprehensive motion dataset that contains necessary motions and transitions. However, in everyday life, we extensively use our arms, hands, and upper body in these interactions. It is difficult to capture all the necessary upper body movement due to the large diversity.
    \item Existing approaches deal with full-body motions. When there are insufficient training data, we can observe coupled upper-body and lower-body movements, making some interactions hard to achieve.
    \item ....
\end{itemize}


In this paper, we present an integrated framework for training and controlling simulated characters with highly flexible upper-body motions. We use a hierarchical control structure with decoupled balance control policies and task-specific upper-body control. It enables useful applications such as reconstructing a user's full-body movement from the input of several VR devices.

Our principal contributions include:
\begin{itemize}
    \item We present an integrated framework that generates upper-body movement and lower-body movement.
    \item We demonstrate successful training of a complicated system with carefully designed training process. (iterative training of control policies)
    \item As an application of the proposed framework, we demonstrated the first data-driven physics-based 3pt tracking system.
    \item
\end{itemize}


